Performance Analysis of Quantum Key Distribution in Underwater Channels

The current literature on quantum key distribution (QKD) is mainly limited to the transmissions over fiber optic, atmospheric or satellite links and are not directly applicable to underwater environments with different channel characteristics. Absorption, scattering, and turbulence experienced in underwater channels severely limit the range of quantum communication links. In the first part of this thesis, we analyze the quantum bit error rate (QBER) and secret key rate (SKR) performance of the well-known BB84 protocol in underwater channels. As path loss model, we consider a modified version of Beer-Lambert formula which takes into account the effect of scattering. We derive a closed-form expression for the wave structure function to determine the average power transfer over turbulent underwater path and use this to obtain an upper bound on QBER as well as a lower bound on SKR. In the second part of this thesis, as a potential solution to overcome range limitations, we investigate a multi-hop underwater QKD where intermediate nodes between the source and destination nodes help the key distribution. We consider the deployment of passive relays which simply redirect the qubits to the next relay node or the receiver without any measurement. Based on the near-field analysis, we present the performance of relay-assisted QKD scheme in terms of QBER and SKR in different water types and turbulence conditions. In the last part of this thesis, we investigate the fundamental performance limits of decoy BB84 protocol over turbulent underwater channels and provide a comprehensive performance characterization. Based on near field analysis, we utilize the wave structure function to determine the average power transfer over turbulent underwater path and use this to obtain a lower bound on key generation rate. Based on this bound, we present the performance of decoy BB84 protocol in different water type.

==> Chapter_3/chapter_three.tex <==
\chapter{Optimal Selection of Receiver Gate Time for QKD in Underwater Channels}\label{ch:gate}


In addition to the performance degradation due to absorption, scattering, and turbulence experienced in underwater channels, the received noise severely limits the range of quantum communication links \cite{p2_14}. The current theoretical and experimental works ignore the effect of receiver parameters on the noise level and their works are built upon heuristic selection of system parameters. 

At the receiver side, Bob employs InGaAs/InP SPADs working in the Geiger mode as the detector. One promising approach in such detectors to mitigate the effect of background noise is to utilize gate mode \cite{p3_13}. The gate time is the period during which the detector is active and able to detect a possible coming signal. Most of the time the SPADs are in off-mode and a narrow gate time is opened only when the signal photons are expected to arrive. Consequently, the noise photons arriving outside the time window can be blocked. The gate not only eliminates noise, but also potentially eliminates signal counts. A narrow time gate requires precise knowledge of the signal photon’s arrival time to reduce the noise while minimally impacting the signal level \cite{p3_14}. Thus, there is trade-off between the number of background photons and the received signal photons where brings the necessity of finding the optimal value of receiver gate time.


In this chapter, we investigate the effect of gating time in the performance of BB84 protocol over underwater channels. As path loss model, we utilize a Monte Carlo simulation based on MCML method to solve radiative transfer equation \cite{p3_15}. We provide a comprehensive simulation results and illustrate the time of arrival (ToA) and angle of arrival (AoA). Based on these results, we design the QKD system and find the optimal vaule for the gate time in the sense of minizing the QBER. 

\section{System Model}\label{P3_sys}
We consider a QKD system employing BB84 protocol for key distribution over a link distance of $L$. 
% This protocol aims to create a secret key between the authorized partners, Alice and Bob, such that eavesdropper (Eve) cannot acquire noteworthy information. Alice prepares a qubit by choosing randomly between two orthogonal bases, i.e., ${0^ \circ }/ + {90^ \circ }$  basis and $ + {45^ \circ }/ - {45^ \circ }$ basis for every bit she wants to send. She selects a random bit value "0" or "1" and uses polarization encoding of photons where polarization of ${0^ \circ }/ - {45^ \circ }$ represents 0 and polarization of $ + {90^ \circ }/ + {45^ \circ }$ represents 1. After travelling over the underwater channel, the received qubit is randomly sent to two detector corresponding to two bases by the beam splitter where half wave plate converts the states $ - {45^ \circ }$ and $ + {45^ \circ }$ to states ${0^ \circ }$ and $ + {90^ \circ }$, and a polarizing splitter redirects it to the corresponding decoder according to the polarization state of the received photon. The secure key between two parties is constructed based on the "sift" events which correspond to the bit intervals in which exactly one of the single-photon avalanche photodiodes (SPADs) registers a count and both Alice and Bob have chosen the same basis.
We assume an ideal single photon transmitter which emits one single photon per pulse. The laser pulse duration influences the key rate and is calculated based on the maximum time for the arrival photons \cite{p3_16}. 
Underwater QKD communication suffers from severe absorption and scattering due to the inevitable photon interactions with the water molecules and other particles in solution and suspension in water. In addition, according to Mie theory, the scattering may change the polarized state of photons which can lead to an increase in the error of information. Fortunately, it has been shown that the polarized states of the received scattered photons remain almost invariant for underwater communications \cite{p3_17, p1_24}. 

Let $\Delta t'$ and $\Delta t$ denote the receiver gate time and the pulse duration, respectively. Beside from the transmitted photons, receiver will collect   background photons on average. This is given by

$$ {n_B} = {{\pi {R_d}A\lambda \Delta \lambda \left( {1 - \cos \left( \Omega  \right)} \right)\Delta t'} \mathord{\left/
 {\vphantom {{\pi {R_d}A\lambda \Delta \lambda \left( {1 - \cos \left( \Omega  \right)} \right)\Delta t'} {\left( {2{h_p}{c_0}} \right)}}} \right.
 \kern-\nulldelimiterspace} {\left( {2{h_p}{c_0}} \right)}} $$
 
where ${R_d}$ is the irradiance of the environment whose primary source is the refracted sunlight from the surface of the water \cite{p1_27}, $A$ is the receiver aperture area, $\lambda $ is the wavelength, $\Delta \lambda $ is the filter spectral width, $\Omega $ is the field of view, ${h_p}$ is Planck’s constant, and ${c_0}$ is the speed of light. In addition to the background noise, the receiver will be subject to an average equivalent dark current count (denoted as ${I_{dc}}$) which induces an ${n_D} = {I_{dc}}\Delta t$ background photons. Therefore, the average number of noise photons reaching each Bob’s detector can be expressed as \cite{p3_20}
  
  $${n_N} = {n_D} + {{{n_B}} \mathord{\left/
 {\vphantom {{{n_B}} 2}} \right.
 \kern-\nulldelimiterspace} 2}$$
 
Let $\gamma $ denote the fraction of received photons. To ensure correct decoding of the received qubits, each Alice and Bob need to sift the bits that are encoded and decoded using the same bases. Sifting process will result in 50\% of correctness due to the deviant selection on bases at both Alice and Bob \cite{p2_22}. QBER is defined as the error rate in the sifted key and can be calculated as \cite{p3_20}
  
  $$QBER = \frac{{{n_N}}}{{{{\gamma {n_S}} \mathord{\left/
 {\vphantom {{\gamma {n_S}} 2}} \right.
 \kern-\nulldelimiterspace} 2} + 2{n_N}}}$$
where the factor of $\frac{1}{2}$ is introduced as a result of sifting process and ${n_S}$ denotes the average photon number of transmitter.

\section{Channel Modelling Approach}\label{P3_channel}
The transmitter is represented as a circle with an initial radius of ${r_0}$ and maximum initial divergence angle of ${\theta _{0,\max }}$ located in $z = 0$ plane. Let $U\left[ {n,m} \right]$ denote the uniform random variable (RV) with a distribution between $n$ and $m$. The initial location of each photon $\left( {x,y,0} \right)$ is specified by $x = {r_0}\cos {\varphi _0}$ and $y = {r_0}\sin {\varphi _0}$ where the azimuthal angle ${\varphi _0}$ is generated based on $U \sim \left[ {0,2\pi } \right]$. The direction $\left( {{\mu _x},{\mu _y},{\mu _z}} \right)$ of the photon can be expressed as ${\mu _x} = \sin {\theta _0}\cos {\varphi _0}$, ${\mu _y} = \sin {\theta _0}\sin {\varphi _0}$ and ${\mu _z} = \cos {\theta _0}$ where the polar angle ${\theta _0}$ is generated according to $U \sim [ - {\theta _{0,\max }},{\theta _{0,\max }}]$. 

The initial weight of the launched photon is considered as 1. The emitted photon travels a random distance before interacting with a particle in the medium. In homogenous water, the geometric path length $\delta $ can be computed with $\delta  =  - {{\ln \left( q \right)} \mathord{\left/
 {\vphantom {{\ln \left( q \right)} {\varsigma \left( \lambda  \right)}}} \right.
 \kern-\nulldelimiterspace} {\varsigma \left( \lambda  \right)}}$ where $q$ is $U\left[ {0,1} \right]$ and $\varsigma \left( \lambda  \right) = \alpha \left( \lambda  \right) + \beta \left( \lambda  \right)$ is the extinction coefficient where $\alpha \left( \lambda  \right)$ and $\beta \left( \lambda  \right)$ respectively denote absorption and scattering coefficients. The photon loses a fraction of its initial weight and is deviated from its starting path as a result of interaction with the particles. Let $w$ and $w'$ denote the photon weight before and after the interaction, respectively. The photon weight can be updated as $w' = w{{\beta \left( \lambda  \right)} \mathord{\left/
 {\vphantom {{\beta \left( \lambda  \right)} {\varsigma \left( \lambda  \right)}}} \right.
 \kern-\nulldelimiterspace} {\varsigma \left( \lambda  \right)}}$.
 
Let $\left( {{{\mu '}_x},{{\mu '}_y},{{\mu '}_z}} \right)$ denote the new propagation direction. For a given azimuthal angle  $\phi $ and scattering angle $\theta $, they can be defined as $${\mu '_x} = {{\left( {{\mu _x}{\mu _z}\cos \phi  - {\mu _y}\sin \phi } \right)\sin \theta } \mathord{\left/
 {\vphantom {{\left( {{\mu _x}{\mu _z}\cos \phi  - {\mu _y}\sin \phi } \right)\sin \theta } {\sqrt {1 - \mu _z^2} }}} \right.
 \kern-\nulldelimiterspace} {\sqrt {1 - \mu _z^2} }} + {\mu _x}\cos \theta, $$ $${\mu '_y} = {{\left( {{\mu _y}{\mu _z}\cos \phi  + {\mu _x}\sin \phi } \right)\sin \theta } \mathord{\left/
 {\vphantom {{\left( {{\mu _y}{\mu _z}\cos \phi  + {\mu _x}\sin \phi } \right)\sin \theta } {\sqrt {1 - \mu _z^2} }}} \right.
 \kern-\nulldelimiterspace} {\sqrt {1 - \mu _z^2} }} + {\mu _y}\cos \theta, $$ 
 and
 $${\mu '_z} =  - \sin \theta \cos \phi \sqrt {1 - \mu _z^2}  + {\mu _z}\cos \theta.$$ The new position of the photon can be therefore updated by $x' = x + {\mu '_x}\delta $, $y' = y + {\mu '_y}\delta $ and $z' = z + {\mu '_z}\delta $. If the photon direction is close to z-axes (i.e., $\left| {{\mu _z}} \right| > 0.9999$), then the new propagation direction can be approximated as ${\mu '_x} \cong \sin \theta \cos \phi $, ${\mu '_y} \cong \sin \theta \cos \phi $ and ${\mu '_z} \cong {{{\mu _z}\cos \phi } \mathord{\left/
 {\vphantom {{{\mu _z}\cos \phi } {\left| {{\mu _z}} \right|}}} \right.
 \kern-\nulldelimiterspace} {\left| {{\mu _z}} \right|}}$.
 
The azimuthal angle $\phi $ is modeled as an RV with a distribution of $U[0,2\pi ]$. The scattering angle $\theta $ can be calculated based on the scattering phase function which provides the angular distribution of light intensity scattered by a particle \cite{p3_15}. The channel characteristics for collimated beams highly depend on the scattering phase function \cite{p3_15}. An RV $\chi $ is generated randomly with a distribution of $U\left[ {0,\pi } \right]$, and then the corresponding $\theta $ can be calculated as $\chi  = \int_0^\theta  {p\left( {\Psi ,a,{g_{\rm{f}}},{g_{\rm{B}}}} \right)\sin \left( \Psi  \right)d\Psi } $ where $p\left( {\Psi ,a,{g_{\rm{f}}},{g_{\rm{B}}}} \right)$ denotes scattering phase function. 

Here, we utilize the two term Henyey–Greenstein (TTHG) model as the scattering phase function which has a better fit with the experimental results \cite{p3_22}. It is defined as ${p_{{\rm{TTHG}}}}\left( {\theta ,a,{g_{\rm{f}}},{g_{\rm{B}}}} \right) = a{p_{{\rm{HG}}}}\left( {\theta ,{g_{\rm{F}}}} \right) + \left( {1 - a} \right){p_{{\rm{HG}}}}\left( {\theta , - {g_{\rm{B}}}} \right)$ where $a$ is the weight of the forward Henyey–Greenstein (HG) phase function, and ${g_{\rm{F}}}$ and ${g_{\rm{B}}}$ are the asymmetry factors for the forward and backward-directed HG phase functions, respectively \cite{p3_22}.   ${p_{{\rm{HG}}}}\left( {\theta ,g} \right)$ is HG function and is given by ${p_{{\rm{HG}}}}\left( {\theta ,g} \right) = {{\left( {1 - {g^2}} \right)} \mathord{\left/
 {\vphantom {{\left( {1 - {g^2}} \right)} {\left[ {2{{\left( {1 + {g^2} - 2g\cos \theta } \right)}^{1.5}}} \right]}}} \right.
 \kern-\nulldelimiterspace} {\left[ {2{{\left( {1 + {g^2} - 2g\cos \theta } \right)}^{1.5}}} \right]}}$. The relationships between $a$, ${g_{\rm{B}}}$, ${g_{\rm{F}}}$, and $\overline {\cos \theta } $ can be expressed as ${g_{\rm{B}}} =  - 0.3061446 + 1.000568{g_{\rm{F}}} - 0.01826338g_{\rm{F}}^2 + 0.03643748g_{\rm{F}}^3$, $a = {{{g_{\rm{B}}}\left( {1 + {g_{\rm{B}}}} \right)} \mathord{\left/
 {\vphantom {{{g_{\rm{B}}}\left( {1 + {g_{\rm{B}}}} \right)} {\left[ {\left( {{g_{\rm{F}}} + {g_{\rm{B}}}} \right)\left( {1 + {g_{\rm{B}}} - {g_{\rm{F}}}} \right)} \right]}}} \right.
 \kern-\nulldelimiterspace} {\left[ {\left( {{g_{\rm{F}}} + {g_{\rm{B}}}} \right)\left( {1 + {g_{\rm{B}}} - {g_{\rm{F}}}} \right)} \right]}}$, and $\overline {\cos \theta }  = a\left( {{g_{\rm{F}}} + {g_{\rm{B}}}} \right) - {g_{\rm{B}}}$ \cite{p3_22}. Using regression on the experimental data, an approximation for $\overline {\cos \theta } $ is obtained as $\overline {\cos \theta }  = {{2\left( {1 - 2B} \right)} \mathord{\left/
 {\vphantom {{2\left( {1 - 2B} \right)} {\left( {2 + B} \right)}}} \right.
 \kern-\nulldelimiterspace} {\left( {2 + B} \right)}}$ where $B = {{{\beta _b}} \mathord{\left/
 {\vphantom {{{\beta _b}} \beta }} \right.
 \kern-\nulldelimiterspace} \beta }$ and ${\beta _b}$ is back scattering coefficient.
 
The cycle of traveling and interacting with particles proceeds until, whether the photon is absorbed or it reaches the receiver plane. The photon is assumed to be absorbed when its weight becomes less than a threshold denoted as ${w_{th}}$. In the case of reaching the receiver plane, the position, angle of arrival (AoA) and time of arrival (ToA) for the scattered photon indicate whether the photon is received or lost. The photon is determined as received if its location is within the radius of the aperture and its azimuthal AoA is less than field of view (FoV) of the receiver. In addition, the ToA of a received photon should be less than the receiver gate time. In a homogeneous medium, the required time for a photon to move a geometric path length of $L'$ can be calculated as \[t = {{L'} \mathord{\left/
 {\vphantom {{L'} {{c_n}}}} \right.
 \kern-\nulldelimiterspace} {{c_n}}} = {{L'n} \mathord{\left/
 {\vphantom {{L'n} {{c_0}}}} \right.
 \kern-\nulldelimiterspace} {{c_0}}}\] where ${c_n}$ is the speed of light in a medium with index of refraction $n$ \cite{p3_12}. To remove the time of flight effect, we define the ToA as $t' = t - {t_0}$ where ${t_0}$ is the arrival time for the straight line distance between the receiver and transmitter.
 
\section{Simulation Results and Discussion}\label{P3_sim}
In this section, we present simulation results. We assume transmitter beam width of ${r_0} = 3$ mm \cite{p3_15}, a maximum beam divergence of ${\theta _{0,\max }} = {20^ \circ }$ \cite{p3_15}, the dark current count rate of ${I_{dc}} = 60$ Hz \cite{p1_27}, filter spectral width of $\Delta \lambda  = 30$ nm \cite{p1_27}, the wavelength of $\lambda  = 532$ nm \cite{p3_15}, the receiver aperture diameter of $d = 20$ cm \cite{p3_15}, an extinction coefficient of $\varsigma  = 0.151\,{{\rm{m}}^{ - 1}}$ \cite{p3_15} (corresponding to clear ocean condition), $\overline {\cos \theta }  = 0.9675$  \cite{p3_15}, a depth of ${z_d} = 100$ m \cite{p1_27}, the asymptotic diffuse attenuation coefficient of ${K_\infty } = 0.08$ \cite{p1_28} and clear atmospheric conditions at night with a full moon, i.e., ${R_d}\left( {\lambda ,0} \right) = {10^{ - 3}}\,{{\rm{W}} \mathord{\left/
 {\vphantom {{\rm{W}} {{{\rm{m}}^{\rm{2}}}}}} \right.
 \kern-\nulldelimiterspace} {{{\rm{m}}^{\rm{2}}}}}$ \cite{p1_29}. In our simulations, we have generated at least $10^7$ photons for each experiment, and have repeated the experiments at least 10 times to obtain reliable results. For the convenience of the reader, the channel and system parameters are summarized in Table \ref{table_p3}.


\begin{table}
\captionsetup{justification=centering}
\caption{System and channel parameters}
\label{table_p3}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{ |l|l|l| } 
 \hline
 \textbf{Parameter} & \textbf{Definition} & \textbf{Numerical Value} \\ \hline
${r_0}$ & \text{Transmitter beam width} & $3$ mm \cite{p3_15} \\ \hline 
${\theta _{0,\max }}$ & \text{Maximum beam divergence} & ${20^ \circ }$ \cite{p3_15} \\ \hline 
$\Delta \lambda$ & \text{Filter spectral width} & $30$ $\rm{nm}$ \cite{p1_27} \\ \hline 
$\lambda$ & \text{Wavelength} & $532$ $\rm{nm}$ \cite{p1_27} \\ \hline 
$d$ & \text{Receiver aperture diameter} & $20$ $\rm{cm}$ \cite{p3_15} \\ \hline 
$I_{dc}$ & \text{Dark current count rate} & $60$ $\rm{Hz}$ \cite{p1_27} \\ \hline 
$K_{\infty}$ & \text{Asymptotic diffuse attenuation coefficient} & $0.08$ $\rm{m^{-1}}$ \cite{p1_28} \\ \hline 
$z_d$ & \text{Depth} & $100$ $\rm{m}$ \cite{p1_27} \\ \hline 
${R_d}\left( {\lambda ,0} \right)$ & \text{Irradiance of the underwater environment at sea surface} & ${10^{ - 3}}\,{{\rm{W}} \mathord{\left/
 {\vphantom {{\rm{W}} {{{\rm{m}}^{\rm{2}}}}}} \right.
 \kern-\nulldelimiterspace} {{{\rm{m}}^{\rm{2}}}}}$ \cite{p1_29} \\ \hline 
$\varsigma$ & \text{Extinction coefficient (clear water)} & $0.151$ $\rm{m^{-1}}$ \cite{p3_15} \\\hline
\end{tabular}}
\end{center}
\end{table}



First, we investigate for the received photons over the link distance of  $L = $ 10, 20, 30 and 40 m to indicate the pulse duration. Fig. \ref{fig:p3_1} illustrates the normalized number of received photons versus the ToA. We have considered an FoV of ${180^ \circ }$ to study the worst case concerning symbol interference. We calculate the pulse duration as the maximum ToA for all the received photons. According to our simulation results, we consider the pulse duration as 20 ns for all link distances under consideration.

\begin{figure}[tb]
\centering
\includegraphics[width=0.7\textwidth]{Chapter_3/test_fig1.eps}
\caption{Normalized number of received photons versus time of arrival for clear ocean and link distance of 10, 20, 30 and 40 m.}
\label{fig:p3_1}
\end{figure}



Next, we study the AoA for the received photons to indicate a proper FoV which can affect the number of received signal photons as well as the average number of background photons. As it can be observed from Fig. \ref{fig:p3_2}, AoA of almost all the received photons have angle of less than ${10^ \circ }$.  As a result, wider FoV just leads to an increase in background noise counts and cannot be beneficial in such a harsh propagation environment.

\begin{figure}[tb]
\centering
\includegraphics[width=0.7\textwidth]{Chapter_3/test_fig2.eps}
\caption{Normalized number of received photons versus angle of arrival for clear ocean and link distance of 10, 20, 30 and 40 m.}
\label{fig:p3_2}
\end{figure}



Fig. \ref{fig:p_3_3} illustrates the effect of gate time on the QBER performance for underwater QKD system. We assume a FoV of $\Omega  = {10^ \circ }$. As seen from previous results, we consider pulse duration of $\Delta t = 20$ ns for all link distances under consideration. As it can be observed from Fig. \ref{fig:p_3_3}, there is trade-off between the average number of background photons and the received photons. Through exhaustive search, we find the optimal value of gate time (in the sense of minizing QBER) as 83, 173, 281 and 415 ps for link distance of 10, 20, 30 and 40 m, respectively. Although longer gate time increases the average number of received photons, it also increases the background noise counts which leads to a degradation in QBER performance. 







\begin{figure}
     \centering
     \begin{subfigure}{0.45\textwidth}
         \centering
         \captionsetup{justification=centering}
         \includegraphics[trim=0cm 0.3cm 0.1cm 0.6cm, clip, width=\linewidth]{Chapter_3/test_fig3a.eps}
         \caption{{}}
         \label{fig:p3_3a}
     \end{subfigure}
     \begin{subfigure}{0.45\textwidth}
         \centering
         \captionsetup{justification=centering}
         \includegraphics[trim=0cm 0.3cm 0.1cm 0.6cm, clip, width=\linewidth]{Chapter_3/test_fig3b.eps}
         \caption{{}}
         \label{fig:fig:p3_3b}
     \end{subfigure}
     \centering
     \begin{subfigure}{0.45\textwidth}
         \centering
         \captionsetup{justification=centering}
         \includegraphics[trim=0cm 0.3cm 0.1cm 0.6cm, clip, width=\linewidth]{Chapter_3/test_fig3c.eps}
         \caption{{}}
         \label{fig:fig:p3_3c}
     \end{subfigure}
     \begin{subfigure}{0.45\textwidth}
         \centering
         \captionsetup{justification=centering}
         \includegraphics[trim=0cm 0.3cm 0.1cm 0.6cm, clip, width=\linewidth]{Chapter_3/test_fig3d.eps}
         \caption{{}}
         \label{fig:fig:p3_3d}
     \end{subfigure}
        \caption{QBER performance with respect to the gate time for clear ocean and link distance of \textbf{(a)} $L$ = 10 m, \textbf{(b)} $L$ = 20 m, \textbf{(c)} $L$ = 30 m and \textbf{(d)} $L$ = 40 m}
        \label{fig:p_3_3}
\end{figure}

